Rethinking Human Evaluation Protocol for Text-to-Video Models: Enhancing Reliability,Reproducibility, and Practicality

Recent text-to-video (T2V) technology advancements, as demonstrated by models such as Gen2, Pika, and Sora, have significantly broadened its applicability and popularity. Despite these strides, evaluating these models poses substantial challenges. Primarily, due to the limitations inherent in automatic metrics, manual evaluation is often considered a superior method for assessing T2V generation. However, existing manual evaluation protocols face reproducibility, reliability, and practicality issues. To address these challenges, this paper introduces the Text-to-Video Human Evaluation (T2VHE) protocol, a comprehensive and standardized protocol for T2V models. The T2VHE protocol includes well-defined metrics, thorough annotator training, and an effective dynamic evaluation module. Experimental results demonstrate that this protocol not only ensures high-quality annotations but can also reduce evaluation costs by nearly 50\%. We will open-source the entire setup of the T2VHE protocol, including the complete protocol workflow, the dynamic evaluation component details, and the annotation interface code. This will help communities establish more sophisticated human assessment protocols.

==> RW_appenidx.tex <==
\section{Automated Evaluation Metrics}
While useful for assessing image diversity and clarity through a pre-trained network, IS may prioritize diversity over quality and carry biases from pre-trained networks \cite{salimans2016improved}. FID, which compares feature representations from real and generated images, enhances sensitivity to image quality but can be influenced by superficial similarities and the quality of the comparison dataset \cite{Heusel2017GANsTB}. FVD, designed for videos, examines temporal consistency and quality but might emphasize temporal over spatial quality \cite{unterthiner2019accurate}. CLIPSIM uses the CLIP model to assess alignment between textual descriptions and generated images, offering a measure for text-to-image synthesis, but its reliance on textual data can introduce language and cultural biases \cite{radford2021learning}.

\section{Benchmark Frameworks}
VBench evaluates video generation across multiple dimensions using tailored prompts and human preference annotations but might lack the diversity needed to cover all real-world scenarios \cite{huang2023vbench}. EvalCrafter integrates 17 objective metrics refined by human opinions with diverse prompts, yet may still exhibit biases due to its limited scope \cite{liu2024evalcrafter}. FETV categorizes text prompts into spatial and temporal attributes, combining manual and automatic evaluations, but might not fully capture the variety of real-world scenarios \cite{liu2023fetv}.

\section{Discussion}
Despite advancements in these metrics and benchmarks, their limitations highlight the need for high-quality human evaluations to capture nuanced visual and contextual quality aspects that automated metrics might miss. This approach helps bridge the gap between algorithmic evaluations and real-world applicability.

==> RW_temp.tex <==
Evaluation metrics for visual generative models can be broadly classified into automated evaluation metrics and benchmark methods. For automated evaluation metrics, the IS assesses image diversity and clarity through a pre-trained network \cite{salimans2016improved}, while the FID compares feature representations from real and generated images, enhancing sensitivity to image quality \cite{Heusel2017GANsTB}. The FVD for videos examines temporal consistency and quality \cite{unterthiner2019accurate}. CLIPSIM uses the CLIP model to assess alignment between textual descriptions and generated images, offering a measure for text-to-image synthesis \cite{radford2021learning}. However, these metrics have limitations: IS may prioritize diversity over quality and carry biases from pre-trained networks. FID, despite improvements, can be influenced by superficial similarities and comparison dataset quality. FVD might emphasize temporal over spatial quality, and CLIPSIM's reliance on textual data can introduce language and cultural biases \cite{otani2023verifiable, liu2023fetv}. For the benchmark frameworks, VBench evaluates video generation across multiple dimensions using tailored prompts and human preference annotations \cite{huang2023vbench}. EvalCrafter integrates 17 objective metrics refined by human opinions with diverse prompts \cite{liu2024evalcrafter}. FETV categorizes text prompts into spatial and temporal attributes, combining manual and automatic evaluations \cite{liu2023fetv}. Despite advancements, these benchmarks still have limitations such that they might lack the diversity needed to cover all real-world scenarios, potentially leading to biases \cite{huang2023vbench, liu2024evalcrafter, liu2023fetv,10148799, wu2024better}.

Given the limitations of these automated metrics and benchmarks，high-quality human evaluations remain crucial. Human evaluations can capture nuanced visual and contextual quality aspects that automated metrics might miss, which helps bridge the gap between algorithmic evaluations and real-world applicability. 

==> tables/drop_count.tex <==


\begin{table}[!ht]

    \centering
    \caption{Number of dropped comparisons during the dynamic evaluation.}
    
    \begin{tabular}{lccc}
        \toprule
        Model 1 & Model 2 & Count\\ 
        \midrule

         Gen2 &  Latte & 230 \\  
        ~ & Videocrafter2 & 219 \\  
        ~ & TF-T2V & 215 \\  
        ~ & Pika & 184 \\  
        Pika & Videocrafter2 & 76 \\  
        ~ & TF-T2V & 65 \\  
        ~ &  Latte & 76 \\  
         Latte & TF-T2V & 19 \\  
        ~ & Videocrafter2 & 12 \\  
        TF-T2V & Videocrafter2 & 20 \\  
        
        \bottomrule
    \end{tabular}
    
\label{count1}
\end{table}


==> tables/drop_count2.tex <==



\begin{table}[!ht]

    \centering
    \caption{Your table caption here}
    \label{count2}
    \begin{tabular}{lccc}
        \toprule
        Model & Total Count\\ 
        \midrule

        Gen2      & 848 \\ 
        Pika     & 401 \\ 
        Latte    & 337 \\ 
        TF-T2V       & 319 \\ 
        Videocrafter2   & 327 \\ 
        
        \bottomrule
    \end{tabular}

\end{table}


==> tables/iaa_lab.tex <==



\begin{table}[!ht]

    \centering
    \caption{Comparison of internal IAA of annotators. We compute Krippendorff’s $\alpha$~\cite{Krippendorff1980ContentAA} as an IAA measure. Higher values represent more consensus among annotators.}
    
    \begin{tabular}{lccc}
        \toprule
        Metric & Pre-training LRAs & Post-training LRAs\\ 
        \midrule

        Video Quality & 0.224 & 0.339 \\ 
        Temporal Quality & 0.178 & 0.288 \\ 
        Motion Quality & 0.164 & 0.321 \\ 
        Text Alignment & 0.145 & 0.236 \\ 
        Ethical Robustness & 0.055 & 0.107 \\ 
        Human Preference & 0.195 & 0.284 \\ 
        
        \bottomrule
    \end{tabular}
\label{iaa_lab}
\end{table}

